OGLE-IV Real-Time Transient Search

We present the design and first results of a real-time search for transients within the 650 sq. deg. area around the Magellanic Clouds, conducted as part of the OGLE-IV project and aimed at detecting supernovae, novae and other events. The average sampling of about 4 days from September to May, yielded a detection of 238 transients in 2012/2013 and 2013/2014 seasons. The superb photometric and astrometric quality of the OGLE data allows for numerous applications of the discovered transients. We use this sample to prepare and train a Machine Learning-based automated classifier for early light curves, which distinguishes major classes of transients with more than 80% of correct answers. Spectroscopically classified 49 supernovae Type Ia are used to construct a Hubble Diagram with statistical scatter of about 0.3 mag and fill the least populated region of the redshifts range in the Union sample. We investigate the influence of host galaxy environments on supernovae statistics and find the mean host extinction of A_I=0.19+-0.10 mag and A_V=0.39+-0.21 mag based on a subsample of supernovae Type Ia. We show that the positional accuracy of the survey is of the order of 0.5 pixels (0.13 arcsec) and that the OGLE-IV Transient Detection System is capable of detecting transients within the nuclei of galaxies. We present a few interesting cases of nuclear transients of unknown type. All data on the OGLE transients are made publicly available to the astronomical community via the OGLE website.

==> table1.tex <==
12-NOVA-02 & SMC714.19.5N & 0:32:55.06 & -74:20:19.7 & 6083.89340 & 11.30 & - & CN & 0.70 & - & - & - & - & - & - & - & - & CN \\
12-NOVA-03 & LMC500.11.11N & 5:20:21.09 & -73:05:43.3 & 6230.75237 & 12.93 & - & CN & 1.00 & - & - & - & - & - & - & - & - & CN \\
12-SN-005 & MBR126.24.184N & 3:00:50.89 & -70:31:11.4 & 6212.79171 & 18.62 & 4481 & Ia & 0.80 & Ia & 0.076 & 4594 & 4.68 & 6.66 & 5.01 & 2.65 & S & Ia \\
12-SN-006 & MBR134.28.15N & 3:33:34.79 & -74:23:40.1 & 6217.74826 & 17.61 & 4495 & Ia & 0.98 & Ibn & 0.06 & 4734 & - & - & - & - & - & Ibn \\
12-SN-007 & MBR124.11.19N & 3:01:13.44 & -75:01:16.1 & 6218.84329 & 18.36 & 4495 & Ia & 1.00 & Ia & 0.059438 & 4602 & - & - & - & - & S & Ia \\
12-SN-008 & LMC537.05.1N & 4:33:37.01 & -71:32:20.4 & 6137.94129 & 18.55 & 4495 & CN & 0.70 & - & - & - & - & - & - & - & Ell & unknown likely Ia \\
12-SN-009 & SMC700.05.8N & 0:13:56.46 & -70:01:41.3 & 6104.93091 & 14.89 & 4495 & Ia & 1.00 & Ia & 0.013966 & 3168 & (23.6) & - & - & - & - & Ia \\
12-SN-010 & MBR122.09.9N & 2:58:26.16 & -72:45:12.0 & 6185.78812 & 18.23 & 4495 & IIn & 0.67 & - & - & - & 0.23 & - & 0.25 & 6.15 & S & Ia \\
12-SN-011 & MBR106.20.8N & 2:08:45.14 & -70:39:00.7 & 6141.86720 & 18.52 & 4495 & Ia & 1.00 & - & - & - & 5.11 & - & 5.23 & 2.64 & S & Ia \\
12-SN-012 & LMC535.26.170N & 4:36:17.61 & -73:09:21.9 & 6195.87036 & 18.66 & 4495 & IIn & 0.67 & - & - & - & 4.19 & - & 6.00 & 2.43 & S & Ia \\
12-SN-013 & LMC551.24.8N & 5:42:48.70 & -71:35:52.5 & 6185.88063 & 18.82 & 4495 & IIn & 0.93 & - & - & - & - & - & - & - & S & IIn \\
12-SN-014 & LMC539.06.1N & 4:37:19.18 & -69:08:25.2 & 6150.92144 & 18.20 & 4495 & Ia & 1.00 & Ia & 0.059 & 3280 & - & - & - & - & S & Ia \\
12-SN-015 & LMC549.30.12N & 4:33:19.02 & -65:07:56.1 & 6147.94098 & 19.05 & 4495 & CN & 0.70 & - & - & - & - & - & - & - & S & unknown \\
12-SN-016 & LMC562.02.1N & 5:58:56.36 & -68:02:54.9 & 6158.89128 & 19.18 & 4495 & CN & 0.70 & - & - & - & 6.29 & - & 6.59 & 2.55 & S & unknown likely II \\
12-SN-017 & MBR128.21.3N & 3:09:20.61 & -73:00:02.6 & 6111.90423 & 19.13 & 4495 & CN & 0.70 & - & 0.062040 & NED & 10.99 & - & 11.39 & 10.36 & S & IIp or IIl \\
12-SN-018 & SMC717.13.18N & 0:53:37.61 & -70:04:01.0 & 6151.81165 & 19.13 & 4495 & Ia & 0.90 & - & - & - & - & - & - & - & S & Ia \\
12-SN-019 & MBR127.02.6N & 3:09:51.27 & -72:15:24.6 & 6160.90569 & 19.26 & 4495 & Ia & 1.00 & - & - & - & 7.77 & - & 11.56 & 12.36 & S & unknown likely II \\
12-SN-020 & SMC714.22.48N & 0:27:08.75 & -74:14:08.2 & 6140.78721 & 18.50 & 4495 & DN & 1.00 & - & 0.062293 & NED & 6.45 & - & 6.88 & 12.87 & S & Ia \\
12-SN-021 & MBR131.29.12N & 3:21:03.26 & -70:51:13.8 & 6159.90800 & 19.18 & 4495 & Ia & 0.90 & - & - & - & 2.77 & - & 3.59 & 3.88 & S & Ia \\
12-SN-022 & MBR133.05.7N & 3:22:32.00 & -74:16:34.6 & 6159.91212 & 19.76 & 4495 & Ia & 0.90 & - & - & - & - & - & - & - & S & IIp \\
12-SN-023 & LMC554.06.6N & 5:40:58.11 & -68:35:09.5 & 6181.88999 & 19.79 & 4495 & Ia & 1.00 & - & - & - & - & - & - & - & Ell & Ia \\
12-SN-024 & LMC532.20.243N & 4:56:00.97 & -68:00:31.2 & 6230.72111 & 19.49 & 4541 & Ia & 0.32 & - & - & - & - & - & - & - & S & IIp \\
12-SN-025 & MBR127.15.13N & 3:00:35.50 & -71:57:21.3 & 6191.84436 & 19.17 & 4541 & Ia & 1.00 & - & - & - & 0.12 & - & 0.12 & 0.73 & S & Ia \\
12-SN-026 & SMC705.06.76N & 0:24:42.60 & -70:37:07.7 & 6234.71349 & 19.21 & 4578 & IIp & 0.92 & - & - & - & 4.57 & - & 5.71 & 2.60 & S & Ia \\
12-SN-027 & SMC738.03.156N & 1:35:11.24 & -73:35:36.7 & 6242.72138 & 19.30 & 4578 & Ia & 1.00 & I(maybe) & 0.07 & 4558 & - & - & - & - & S & I \\
12-SN-028 & MBR119.09.18N & 2:48:21.42 & -74:26:40.0 & 6237.78721 & 19.75 & 4578 & IIp & 0.92 & - & - & - & - & - & - & - & S & Ia \\
12-SN-029 & MBR132.10.17N & 3:25:33.65 & -72:44:37.8 & 6237.81540 & 19.57 & 4578 & Ia & 0.79 & - & - & - & 0.74 & - & 0.83 & 2.08 & S & Ia \\
12-SN-030 & LMC547.20.71N & 4:31:51.85 & -67:56:47.9 & 6239.84822 & 18.76 & 4578 & Ia & 1.00 & - & 0.066509 & NED & 3.91 & - & 4.18 & 2.08 & S & Ia \\
12-SN-031 & LMC515.15.153N & 5:27:42.45 & -71:15:50.6 & 6243.81787 & 19.87 & 4578 & Ia & 1.00 & - & - & - & - & - & - & - & S & Ia \\
12-SN-032 & LMC506.02.16N & 5:22:08.05 & -66:09:47.2 & 6248.81761 & 18.73 & 4578 & Ia & 1.00 & Ia & 0.063 & 4602 & - & - & - & - & Ell & Ia \\
12-SN-033 & LMC555.12.119N & 5:43:19.40 & -67:04:21.0 & 6245.78759 & 20.09 & 4578 & Ia & 1.00 & - & - & - & - & - & - & - & - & unknown \\
12-SN-034 & LMC522.23.9N & 4:21:17.75 & -74:38:04.7 & 6246.78692 & 19.93 & 4604 & IIp & 0.70 & - & - & - & - & - & - & - & S & unknown \\
12-SN-035 & LMC574.23.5N & 5:16:44.86 & -62:59:03.5 & 6253.81142 & 19.48 & 4604 & IIp & 0.48 & - & - & - & 6.60 & - & 6.67 & 4.19 & S & unknown \\
12-SN-036 & LMC606.01.2N & 6:15:42.01 & -64:08:57.9 & 6247.82342 & 18.75 & 4604 & IIp & 0.48 & - & - & - & 3.77 & - & 7.00 & 4.71 & S & Ia \\
12-SN-037 & LMC611.14.4N & 6:21:27.72 & -70:05:48.5 & 6158.91761 & 19.56 & 4604 & CN & 0.70 & - & - & - & 5.07 & 3.59 & 7.73 & 7.05 & S & unknown likely II \\
12-SN-038 & LMC561.22.79N & 5:55:53.05 & -68:28:43.5 & 6249.76224 & 19.96 & 4604 & IIp & 0.70 & - & - & - & 8.78 & - & 10.35 & 7.21 & S & unknown \\
12-SN-039 & LMC612.20.18N & 6:29:40.49 & -70:55:36.0 & 6252.84831 & 20.02 & 4604 & IIp & 0.70 & - & - & - & 4.06 & - & 5.82 & 2.74 & S & unknown \\
12-SN-040 & LMC568.14.15N & 6:07:01.59 & -69:21:17.1 & 6264.81780 & 15.95 & 4604 & Ia & 1.00 & Ia & 0.014690 & 4618 & 0.76 & 0.22 & 0.76 & 3.93 & Ell & Ia \\
12-SN-041 & LMC538.10.26N & 4:42:23.37 & -70:05:46.3 & 6264.76484 & 19.79 & 4641 & Ia & 0.30 & - & - & - & - & - & - & - & S & unknown \\
12-SN-042 & LMC595.07.4N & 5:25:27.44 & -60:24:35.8 & 6246.76639 & 18.66 & 4641 & IIn & 0.67 & - & - & - & 7.52 & - & 7.52 & 2.71 & S & unknown likely II \\
12-SN-043 & LMC576.24.6N & 5:15:38.11 & -60:36:06.4 & 6266.82530 & 19.07 & 4641 & Ia & 0.99 & - & - & - & - & - & - & - & S & Ia \\
12-SN-044 & LMC576.32.362N & 5:14:53.48 & -60:08:47.7 & 6276.79792 & 18.42 & 4641 & Ia & 1.00 & Ia & 0.06 & 4734 & - & - & - & - & S & Ia \\
12-SN-045 & LMC580.19.9N & 5:11:28.24 & -61:08:29.7 & 6285.75809 & 19.66 & 4657 & Ia & 0.90 & - & - & - & - & - & - & - & - & unknown \\
12-SN-046 & LMC595.28.7N & 5:29:47.99 & -59:29:59.4 & 6277.82714 & 19.27 & 4657 & Ia & 0.90 & Ia & 0.111 & 4734 & 1.69 & 3.37 & 2.53 & 0.91 & S & Ia \\
12-SN-047 & MBR144.11.34N & 4:04:14.25 & -75:12:08.2 & 6263.72945 & 19.67 & 4657 & Ia & 0.36 & - & - & - & 1.16 & - & 1.51 & 0.76 & S & Ia \\
12-SN-048 & SMC732.19.38N & 1:23:14.23 & -72:19:54.7 & 6297.58574 & 18.37 & 4676 & IIn & 0.67 & IIn & 0.067 & 4696 & 3.58 & 4.54 & 3.82 & 3.88 & S & IIn \\
12-SN-049 & SMC711.14.32N & 0:37:48.09 & -70:44:46.5 & 6285.58220 & 18.65 & 4676 & IIn & 0.67 & Ia & 0.07 & 4696 & - & - & - & - & S & Ia \\
12-SN-050 & LMC564.04.23N & 5:52:34.36 & -65:26:59.7 & 6311.71617 & 18.19 & 4689 & IIn & 0.97 & IIn & 0.082 & 4696 & 3.56 & 5.43 & 3.58 & 2.04 & S & IIn \\
12-SN-051 & LMC578.24.12N & 5:04:06.71 & -63:34:57.0 & 6290.78024 & 19.73 & 4689 & Ia & 0.90 & Ia & 0.11 & 4698 & 6.32 & 12.52 & 6.90 & 2.22 & S & Ia \\
12-SN-052 & LMC599.23.6N & 5:36:29.34 & -60:28:37.5 & 6255.80414 & 18.97 & 4690 & IIp & 0.48 & - & - & - & 0.28 & - & 0.42 & 3.62 & S & Ia \\
13-SN-001 & SMC797.03.426N & 0:46:30.44 & -65:08:16.4 & 6297.55517 & 18.83 & 4718 & IIp & 0.48 & Ia & 0.09 & 4721 & - & - & - & - & S & Ia \\
13-SN-002 & SMC810.26.1800N & 1:23:30.46 & -64:39:42.9 & 6301.57563 & 18.52 & 4718 & IIn & 0.67 & II & 0.0722 & 4721 & 1.10 & 1.49 & 1.17 & 1.72 & S & IIn \\
13-SN-003 & SMC743.13.16N & 23:15:46.39 & -76:58:17.1 & 6263.59832 & 18.43 & 4718 & Ia & 0.46 & - & - & - & 0.09 & - & 0.10 & 3.47 & S & unknown likely nuclear \\
13-SN-004 & SMC769.06.26N & 23:53:52.50 & -79:46:19.0 & 6287.59400 & 18.61 & 4718 & Ia & 1.00 & Ia & 0.06 & 4734 & 13.20 & 15.11 & 13.89 & 4.62 & S & Ia \\
13-SN-005 & SMC799.18.93N & 1:01:37.14 & -67:18:01.7 & 6258.59090 & 19.68 & 4718 & IIp & 0.48 & II & 0.07 & 4734 & - & - & - & - & S & IIp \\
13-SN-006 & SMC800.03.333N & 0:58:08.06 & -66:48:26.7 & 6271.54521 & 19.44 & 4718 & Ia & 0.90 & - & 0.069548 & NED & (24.7) & - & - & - & - & unknown \\
13-SN-007 & SMC805.29.180N & 1:07:56.84 & -65:09:14.4 & 6290.63757 & 19.24 & 4718 & IIp & 0.92 & - & - & - & 16.64 & - & 16.72 & 5.32 & - & unknown likely Ia \\
13-SN-008 & SMC813.32.1389N & 1:30:57.95 & -67:39:12.4 & 6237.66789 & 18.82 & 4718 & Ia & 1.00 & - & - & - & 2.63 & - & 4.25 & 2.85 & S & Ia \\
13-SN-009 & LMC549.03.218N & 4:36:08.21 & -66:09:41.2 & 6296.74994 & 18.67 & 4746 & Ia & 1.00 & Ia & 0.060 & 4734 & 2.20 & 2.52 & 2.20 & 2.79 & S & Ia \\
13-SN-010 & MBR142.13.82N & 3:49:19.65 & -72:33:34.6 & 6309.61450 & 19.26 & 4746 & IIp & 0.48 & - & - & - & - & - & - & - & S & Ia \\
13-SN-011 & LMC586.12.12N & 4:47:10.92 & -64:02:36.5 & 6319.65283 & 18.83 & 4746 & IIp & 0.48 & IIP & 0.05 & 4754 & 5.00 & 4.82 & 5.04 & 3.07 & S & IIP \\
13-SN-012 & LMC512.27.28N & 5:09:52.38 & -65:39:48.6 & 6319.62598 & 19.07 & - & IIn & 0.93 & IIn & 0.08 & 4774 & - & - & - & - & Ell & IIn \\
13-SN-013 & MBR141.02.36N & 3:53:38.01 & -71:45:32.3 & 6309.61246 & 19.15 & 4825 & Ia & 1.00 & - & - & - & - & - & - & - & - & Ia \\
13-SN-014 & MBR141.11.46N & 3:53:07.78 & -71:20:46.6 & 6334.61410 & 17.60 & 4825 & Ia & 0.80 & II & 0.037 & 4829 & 1.03 & 0.75 & 1.11 & 2.35 & S & IIp \\
13-SN-015 & MBR155.18.157N & 2:02:21.55 & -65:44:08.4 & 6338.53517 & 19.38 & 4825 & Ia & 1.00 & Ia & 0.088 & 4829 & - & - & - & - & S & Ia \\
13-SN-016 & LMC581.08.1389 & 5:13:52.76 & -60:09:26.9 & 6379.55018 & 18.68 & 4859 & IIp & 1.00 & IIn & 0.074 & 4860 & - & - & - & - & AGN & IIn \\
13-SN-017 & LMC522.21.1824 & 4:27:22.20 & -74:42:09.4 & 6352.58671 & 18.27 & 4859 & DN & 1.00 & IIn & 0.043 & 4863 & 3.44 & 2.87 & 4.45 & 5.66 & S & IIn \\
13-SN-018 & LMC540.23.45N & 4:39:13.81 & -67:23:36.4 & 6354.57519 & 18.98 & 4875 & Ia & 0.36 & Ia & 0.067 & 4880 & 0.14 & 0.17 & 0.21 & 2.12 & S & Ia \\
13-SN-019 & MBR114.11.509 & 2:27:33.91 & -75:08:16.0 & 6363.50225 & 19.48 & 4875 & Ia & 0.94 & IIn & 0.079 & 4876 & - & - & - & - & S & IIP \\
13-SN-020 & LMC575.15.23N & 5:15:17.87 & -62:00:44.5 & 6354.62311 & 19.51 & 4917 & Ia & 1.00 & - & - & - & 1.94 & - & 3.31 & 3.59 & S & Ia \\
13-SN-021 & LMC519.14.219N & 5:28:01.18 & -66:30:09.0 & 6363.54948 & 18.71 & 4917 & Ia & 0.90 & - & - & - & - & - & - & - & Ell & Ia \\
13-SN-022 & MBR121.29.878 & 2:50:17.36 & -70:52:27.8 & 6369.51506 & 20.01 & 4917 & Ia & 0.98 & - & - & - & 3.30 & - & 4.55 & 2.65 & S & unknown \\
13-SN-023 & LMC552.07.190N & 5:41:43.68 & -70:56:22.7 & 6375.58726 & 19.82 & 4917 & Ia & 0.98 & - & - & - & - & - & - & - & - & unknown \\
13-SN-024 & LMC510.26.4702N & 5:10:48.57 & -68:16:23.8 & 6347.59765 & 19.50 & 4917 & Ia & 1.00 & - & - & - & - & - & - & - & S & Ia \\
13-SN-025 & LMC606.27.276 & 6:13:53.98 & -63:21:25.4 & 6389.55255 & 18.80 & 5000 & Ia & 0.90 & - & - & - & 0.19 & - & 0.19 & 4.66 & S & unknown likely Ia \\
13-SN-026 & SMC723.10.22N & 1:13:38.51 & -69:32:11.4 & 6438.86809 & 19.26 & 5166 & IIp & 0.48 & - & - & - & 1.52 & - & 2.50 & 1.31 & S & unknown \\
13-SN-027 & SMC714.14.62N & 0:22:59.80 & -74:38:32.3 & 6459.94906 & 18.70 & 5166 & IIp & 0.48 & - & - & - & 0.14 & - & 0.16 & 1.69 & S & unknown \\
13-SN-028 & SMC789.27.52N & 0:25:34.22 & -62:54:52.2 & 6438.90375 & 19.73 & 5166 & IIp & 0.48 & - & 0.034300 & NED & 4.10 & - & 4.92 & 7.50 & S & unknown likely II \\
13-SN-029 & SMC714.26.7746 & 0:36:16.30 & -73:59:57.7 & 6467.85673 & 18.77 & 5166 & IIp & 0.92 & - & - & - & 3.20 & - & 3.55 & 3.48 & S & unknown likely Ia \\
13-SN-030 & SMC814.30.44N & 1:32:41.37 & -66:25:43.3 & 6464.93131 & 18.83 & 5204 & IIp & 0.48 & - & - & - & 0.73 & - & 0.93 & 0.72 & - & Ia \\
13-SN-031 & SMC813.22.123 & 1:33:51.35 & -68:07:57.5 & 6464.92926 & 19.68 & 5204 & CN & 0.70 & - & - & - & - & - & - & - & S & unknown \\
13-SN-032 & SMC787.30.67N & 0:19:17.49 & -65:24:42.6 & 6480.93958 & 19.26 & 5204 & Ia & 0.90 & Ia & 0.09 & 5233 & 10.20 & 16.91 & 10.50 & 2.80 & S & Ia \\
13-SN-033 & SMC743.30.2N & 23:16:01.84 & -76:21:09.9 & 6474.90090 & 19.07 & 5204 & IIp & 0.45 & - & - & - & 0.17 & - & 0.18 & 4.14 & S & unknown nuclear \\
13-SN-034 & SMC702.29.613 & 0:10:47.75 & -71:28:28.2 & 6482.92392 & 19.68 & 5204 & Ia & 0.90 & - & - & - & 1.62 & - & 1.78 & 7.90 & S & Ia \\
13-SN-035 & MBR153.24.65N & 1:58:24.30 & -67:55:54.5 & 6479.95207 & 18.91 & 5220 & IIp & 0.48 & - & - & - & 0.91 & - & 1.84 & 2.45 & S & unknown likely II \\
13-SN-036 & SMC716.22.274N & 0:54:27.93 & -68:37:30.7 & 6483.85725 & 19.08 & 5220 & Ia & 0.36 & - & - & - & 1.76 & - & 2.25 & 2.33 & S & Ia \\
13-SN-037 & SMC808.14.42N & 1:18:00.44 & -67:43:16.3 & 6487.90527 & 19.88 & 5220 & IIn & 0.53 & - & - & - & 0.09 & - & 0.12 & 1.84 & S & AGN-flare \\
13-SN-038 & SMC751.09.55N & 23:39:24.77 & -67:02:54.8 & 6494.70677 & 17.97 & 5235 & IIn & 0.67 & II & 0.045 & 5249 & - & - & - & - & S & Unknown \\
13-SN-039 & SMC707.04.24N & 0:22:33.02 & -72:53:41.9 & 6494.76434 & 18.94 & 5235 & Ia & 0.90 & Ia & 0.08 & 5233 & 2.22 & 3.31 & 3.10 & 3.47 & S & Ia \\
13-SN-040 & SMC802.23.63N & 0:53:49.35 & -63:49:24.1 & 6508.81760 & 19.25 & 5251 & Ia & 0.80 & Ia & 0.09 & 5250 & 1.22 & 2.03 & 1.49 & 1.41 & S & Ia \\
13-SN-041 & SMC812.13.110N & 1:36:17.96 & -69:34:12.5 & 6508.83856 & 19.44 & 5251 & Ia & 1.00 & Ia & 0.10 & 5250 & 2.39 & 4.36 & 2.42 & 3.35 & S & Ia \\
13-SN-042 & SMC706.06.7602 & 0:23:16.85 & -71:42:49.2 & 6507.85177 & 19.82 & 5251 & Ia & 1.00 & - & - & - & 0.69 & - & 0.69 & 1.37 & S & Ia \\
13-SN-043 & SMC800.23.1047 & 0:52:48.79 & -66:09:48.6 & 6508.81269 & 20.27 & 5251 & IIp & 0.70 & Ia & 0.14 & 5290 & 2.29 & 5.60 & 2.49 & 2.02 & S & Ia \\
13-SN-044 & SMC820.14.61N & 0:18:50.31 & -77:33:32.6 & 6511.78989 & 18.75 & 5277 & Ia & 0.90 & Ia & 0.07 & 5284 & 0.99 & 1.31 & 1.03 & 1.75 & S & Ia \\
13-SN-045 & SMC753.19.44N & 23:40:36.52 & -64:17:22.6 & 6515.81102 & 20.03 & 5277 & IIp & 0.70 & II & 0.10 & 5290 & - & - & - & - & - & IIP \\
13-SN-046 & SMC804.05.88N & 1:07:29.73 & -67:26:03.6 & 6514.80302 & 19.66 & 5277 & Ia & 0.90 & II & 0.07 & 5290 & - & - & - & - & S & IIP \\
13-SN-047 & SMC753.19.43N & 23:40:35.48 & -64:24:22.7 & 6515.81102 & 18.35 & 5277 & Ia & 1.00 & II & 0.06 & 5284 & 1.40 & 1.60 & 1.86 & 2.61 & - & IIP \\
13-SN-048 & SMC813.11.50N & 1:37:10.25 & -68:23:48.6 & 6519.75978 & 19.77 & 5292 & IIn & 0.53 & II & 0.06 & 5290 & 1.75 & 2.00 & 2.89 & 1.94 & S & IIP \\
13-SN-049 & MBR138.13.114N & 3:36:04.02 & -73:09:11.5 & 6519.86362 & 18.51 & 5292 & IIn & 0.67 & - & - & - & - & - & - & - & S & AGN-flare \\
13-SN-050 & SMC793.20.1N & 0:36:11.73 & -63:45:36.5 & 6520.71662 & 19.00 & 5292 & Ia & 0.32 & unkn & 0.13 & 5338 & 0.09 & 0.22 & 0.10 & 2.95 & S & GalaxyAGN \\
13-SN-051 & SMC791.12.33N & 0:32:19.55 & -66:25:44.3 & 6520.71233 & 18.73 & 5292 & Ia & 0.90 & Ia & 0.07 & 5335 & 1.80 & 2.38 & 1.81 & 1.98 & S & Ia \\
13-SN-052 & MBR118.20.216N & 2:39:53.91 & -73:07:05.3 & 6520.87379 & 19.48 & 5292 & Ia & 1.00 & - & - & - & 12.29 & - & 17.29 & 5.32 & S & Ia \\
13-SN-053 & MBR117.15.46N & 2:29:49.33 & -71:57:45.2 & 6520.87173 & 19.18 & 5321 & Ia & 1.00 & - & - & - & 0.89 & - & 1.77 & 2.98 & S & Ia \\
13-SN-054 & MBR122.04.597 & 2:51:33.57 & -73:00:49.3 & 6521.77577 & 19.83 & 5321 & Ia & 1.00 & - & - & - & 0.86 & - & 0.86 & 1.44 & S & Ia \\
13-SN-055 & SMC702.29.613 & 0:10:47.75 & -71:28:28.2 & 0.00000 & 19.68 & 5321 & Ia & 0.90 & - & - & - & - & - & - & - & S & Ia \\
13-SN-056 & LMC583.23.313 & 4:55:34.55 & -63:05:31.2 & 6522.93175 & 20.44 & 5321 & Ia & 0.94 & - & - & - & 0.13 & - & 0.16 & 1.54 & S & unknown \\
13-SN-057 & SMC793.02.42N & 0:37:02.41 & -64:29:50.0 & 6531.83447 & 19.40 & 5368 & IIp & 0.48 & Ia & 0.10 & 5345 & 1.25 & 2.28 & 1.28 & 1.45 & S & Ia \\
13-SN-058 & MBR200.11.30N & 2:51:13.59 & -63:59:33.8 & 6531.88532 & 17.61 & 5368 & CN & 0.70 & - & - & - & 7.11 & - & 8.98 & 4.01 & S & unknown-likelyIIn \\
13-SN-059 & MBR202.13.2N & 3:03:11.21 & -68:27:39.8 & 6526.81470 & 18.72 & 5368 & IIp & 0.45 & - & - & - & - & - & - & - & S & AGN \\
13-SN-060 & LMC602.04.31N & 5:48:11.18 & -61:42:15.4 & 6538.90401 & 18.63 & 5368 & Ia & 0.80 & - & - & - & - & - & - & - & S & Ia \\
13-SN-061 & LMC575.18.398 & 5:22:33.54 & -61:53:54.8 & 6533.89871 & 19.96 & 5368 & IIn & 0.53 & - & - & - & 1.23 & - & 1.36 & 5.78 & S & unknown \\
13-SN-062 & LMC601.20.1216 & 5:50:53.43 & -62:24:43.8 & 6538.90194 & 19.26 & 5368 & Ia & 0.36 & - & - & - & 0.29 & - & 0.30 & 1.14 & S & Ia \\
13-SN-063 & MBR203.14.488 & 3:01:54.01 & -67:07:49.6 & 6537.86792 & 19.63 & 5368 & IIp & 0.48 & - & - & - & - & - & - & - & - & IIp \\
13-SN-064 & MBR207.03.928 & 3:21:53.46 & -70:29:46.1 & 6537.87613 & 18.48 & 5368 & IIn & 0.67 & - & - & - & 2.99 & - & 3.00 & 3.27 & S & Ia \\
13-SN-065 & SMC824.07.741 & 0:56:40.86 & -80:16:33.3 & 6537.80629 & 19.68 & 5368 & IIp & 0.48 & - & - & - & 0.47 & - & 0.49 & 1.17 & S & unknown \\
13-SN-066 & LMC622.22.4N & 4:26:10.28 & -62:31:07.0 & 6543.92258 & 17.66 & 5397 & Ia & 0.80 & - & 0.017509 & NED & 0.22 & - & 0.24 & 3.91 & S & AGN \\
13-SN-067 & MBR135.28.39N & 3:39:46.50 & -75:47:33.6 & 6545.81138 & 19.83 & 5397 & IIn & 0.53 & - & - & - & 7.62 & - & 7.95 & 8.51 & S & unknown-likelyIIp \\
13-SN-068 & LMC517.03.1385N & 5:34:00.16 & -69:03:06.1 & 6547.87983 & 19.12 & 5397 & Ia & 0.36 & - & - & - & - & - & - & - & S & unknown-likelyIIn \\
13-SN-069 & SMC811.31.1104N & 1:15:50.70 & -63:17:17.3 & 6543.82157 & 19.97 & 5397 & IIn & 0.53 & - & - & - & - & - & - & - & S & IIp \\
13-SN-070 & SMC796.04.44N & 0:45:14.41 & -66:19:50.6 & 6545.75057 & 17.89 & 5397 & Ia & 1.00 & Ia & 0.043 & 5455 & - & - & - & - & - & Ia \\
13-NOVA-01 & MBR220.01.13N & 3:55:06.25 & -69:23:40.9 & 6523.83008 & 14.69 & - & CN & 1.00 & - & - & - & - & - & - & - & - & CN \\
13-SN-071 & LMC520.15.10585 & 5:26:09.30 & -65:08:13.4 & 6548.86404 & 19.13 & 5397 & IIp & 0.48 & - & - & - & 0.21 & - & 0.23 & 7.34 & S & unknown \\
13-SN-072 & MBR226.15.30N & 3:59:37.66 & -69:29:26.6 & 6546.86585 & 19.32 & 5445 & IIp & 1.00 & - & - & - & 0.31 & - & 0.33 & 7.10 & AGN & AGN-flare \\
13-SN-073 & MBR118.09.63N & 2:44:54.81 & -73:20:35.8 & 6564.71252 & 19.05 & 5445 & Ia & 0.90 & Ia & 0.091 & 5400 & 4.46 & 7.47 & 4.69 & 5.29 & S & Ia \\
13-SN-074 & MBR121.06.54N & 2:47:14.24 & -71:49:32.0 & 6563.74401 & 18.77 & 5445 & IIp & 0.48 & - & - & - & 2.56 & - & 5.71 & 6.67 & S & unknown \\
13-SN-075 & MBR153.07.76N & 1:58:01.88 & -68:45:47.9 & 6565.85535 & 18.95 & 5445 & Ia & 0.90 & Ia & 0.08 & 5440 & 4.67 & 6.97 & 6.02 & 4.55 & S & Ia \\
13-SN-076 & LMC555.32.3252N & 5:38:31.91 & -66:29:38.9 & 6561.85555 & 18.02 & 5445 & IIn & 0.97 & - & - & - & - & - & - & - & S & IIn \\
13-SN-077 & MBR179.21.47N & 2:08:49.55 & -67:22:50.5 & 6563.75965 & 20.58 & 5445 & IIp & 0.42 & - & - & - & - & - & - & - & - & unknown \\
13-SN-078 & SMC739.06.52N & 1:26:31.49 & -74:44:53.1 & 6565.66621 & 19.12 & 5445 & DN & 1.00 & - & - & - & 3.79 & - & 3.80 & 2.76 & AGN & Ia \\
13-SN-079 & SMC790.09.68N & 0:35:10.20 & -67:41:08.5 & 6565.68692 & 19.81 & 5445 & Ia & 1.00 & I & 0 & 5443 & - & - & - & - & S & unknown \\
13-SN-080 & SMC735.14.52N & 1:02:33.24 & -76:27:24.2 & 6565.65763 & 19.60 & 5445 & Ia & 0.99 & Ia & 0.103 & 5443 & 3.80 & 7.11 & 3.95 & 2.36 & S & Ia \\
13-SN-081 & LMC677.06.13N & 8:11:38.05 & -70:57:43.5 & 6562.88325 & 18.90 & 5455 & - & - & - & - & - & - & - & - & - & S & - \\
13-SN-082 & LMC549.01.26N & 4:38:39.51 & -66:13:58.2 & 6567.89397 & 18.55 & 5488 & IIn & 0.67 & - & 0.048867 & NED & - & - & - & - & S & AGN-flare \\
13-SN-083 & MBR110.12.51N & 2:05:48.86 & -75:42:26.2 & 6569.74423 & 20.37 & 5488 & IIp & 0.45 & - & - & - & - & - & - & - & S & unknown \\
13-SN-084 & MBR118.02.78N & 2:41:49.12 & -73:27:52.5 & 6569.76567 & 19.71 & 5488 & IIp & 1.00 & - & - & - & 7.08 & - & 7.12 & 5.03 & S & Ia \\
13-SN-085 & MBR187.22.207N & 2:18:14.52 & -64:56:59.6 & 6568.83820 & 19.25 & 5488 & Ia & 1.00 & - & - & - & 0.57 & - & 0.66 & 3.16 & S & Ia \\
13-SN-086 & SMC797.20.360N & 0:46:36.36 & -64:31:06.7 & 6569.69769 & 20.35 & 5488 & Ia & 0.97 & - & - & - & 5.33 & - & 5.42 & 7.01 & S & unknown \\
13-SN-087 & LMC534.12.38N & 4:55:44.52 & -65:40:27.8 & 6571.87145 & 19.71 & 5488 & Ia & 0.36 & - & - & - & 4.62 & - & 5.52 & 1.70 & Ell & unknown \\
13-SN-088 & LMC548.07.41N & 4:27:44.75 & -67:24:22.4 & 6573.79563 & 19.59 & 5488 & IIp & 0.48 & AGN & 0.168 & 5459 & - & - & - & - & AGN & AGN \\
13-SN-089 & LMC599.26.1289N & 5:42:37.14 & -60:09:12.2 & 6572.84328 & 19.47 & 5488 & IIp & 0.48 & - & - & - & 6.36 & - & 6.71 & 5.13 & S & unknown \\
13-SN-090 & MBR229.10.1N & 4:08:38.82 & -65:45:59.2 & 6571.75868 & 18.64 & 5488 & Ia & 0.80 & AGN & 0.125 & 5537 & 0.10 & 0.23 & 0.11 & 5.45 & AGN & AGN \\
13-SN-091 & LMC596.26.1733N & 5:44:44.23 & -63:55:51.1 & 6575.87438 & 18.51 & 5488 & Ia & 0.80 & Ic & 0.08 & 5510 & 6.32 & 9.42 & 7.67 & 9.22 & Ell & Ic \\
13-SN-092 & SMC742.20.305N & 23:17:21.63 & -77:53:55.5 & 6572.62264 & 20.13 & 5488 & Ia & 1.00 & - & - & - & - & - & - & - & - & Ia \\
13-SN-093 & LMC503.19.415N & 5:23:09.14 & -69:03:46.2 & 6571.84517 & 19.81 & 5488 & Ia & 0.36 & - & - & - & - & - & - & - & S & Ia \\
13-SN-094 & LMC644.05.41N & 5:34:48.25 & -76:38:39.8 & 6573.80699 & 19.52 & 5488 & Ia & 1.00 & - & - & - & 0.47 & - & 0.52 & 1.10 & S & unknown \\
13-NOVA-02 & LMC649.28.33N & 5:57:58.35 & -74:54:08.9 & 6771.49064 & 11.55 & - & CN & 0.90 & - & - & - & - & - & - & - & - & CN \\
13-SN-095 & LMC657.18.66N & 6:43:01.30 & -76:25:11.2 & 6584.87665 & 18.77 & 5497 & DN & 1.00 & - & - & - & - & - & - & - & S & DN \\
13-SN-096 & LMC599.20.159N & 5:39:38.80 & -60:39:32.1 & 6584.78940 & 19.60 & 5497 & Ia & 0.90 & Ia & 0.11 & 5510 & 5.89 & 11.68 & 8.01 & 4.60 & S & Ia \\
13-SN-097 & LMC548.19.44N & 4:34:33.92 & -66:46:42.7 & 6584.83860 & 19.77 & 5497 & Ia & 0.90 & - & - & - & 1.87 & - & 2.54 & 14.39 & S & unknown \\
13-SN-098 & LMC712.04.7N & 5:26:36.40 & -49:28:03.9 & 6583.86939 & 18.70 & 5497 & Ia & 0.90 & Ia & 0.06 & 5504 & 1.15 & 1.32 & 1.50 & 3.99 & S & Ia \\
13-SN-099 & LMC676.12.15N & 8:02:27.32 & -72:25:26.6 & 6585.87341 & 17.71 & 5497 & Ia & 1.00 & Ia & 0.028 & 550 & 3.71 & 2.06 & 4.35 & 7.84 & S & Ia \\
13-SN-100 & MBR114.24.1106 & 2:16:18.56 & -74:45:23.7 & 6586.67071 & 18.89 & 5497 & IIp & 0.48 & II-pec & 0.09 & 5617 & 1.05 & 1.74 & 1.11 & 2.57 & S & uknown-peculiar \\
13-SN-101 & LMC579.20.639 & 5:10:10.57 & -62:31:29.2 & 6584.76180 & 19.84 & 5497 & IIp & 0.70 & - & - & - & 2.29 & - & 2.90 & 3.78 & S & uknown \\
13-SN-102 & LMC644.24.2119 & 5:31:12.75 & -75:50:49.6 & 6584.84950 & 19.11 & 5497 & IIp & 0.70 & - & - & - & 0.00 & - & 0.01 & 0.44 & - & unknown-likely DN \\
13-SN-103 & MBR121.06.808 & 2:46:12.84 & -71:50:45.0 & 6585.75997 & 18.71 & 5497 & IIp & 0.48 & - & - & - & 2.10 & - & 2.48 & 2.53 & S & Unknown/I/IIb \\
13-SN-104 & MBR171.22.812 & 3:22:00.48 & -76:34:11.6 & 6586.69717 & 19.15 & 5497 & Ia & 1.00 & - & - & - & 0.19 & - & 0.21 & 2.24 & S & Ia \\
13-SN-105 & MBR213.27.331 & 3:38:44.20 & -69:06:01.4 & 6585.77689 & 19.80 & 5497 & Ia & 0.90 & - & 0.051479 & NED & 14.89 & - & 14.92 & 9.04 & S & unknown \\
13-SN-106 & SMC770.06.363 & 23:53:06.84 & -78:33:19.5 & 6583.58641 & 19.30 & 5497 & Ia & 0.98 & - & - & - & 1.20 & - & 1.44 & 2.20 & S & Ia \\
13-SN-107 & SMC787.23.110N & 0:17:38.87 & -65:39:34.8 & 6595.60489 & 19.84 & 5535 & Ia & 1.00 & - & - & - & - & - & - & - & - & Ia \\
13-SN-108 & SMC784.27.66N & 0:14:10.58 & -63:19:31.2 & 6595.59871 & 18.90 & 5535 & IIn & 0.42 & - & - & - & 0.46 & - & 0.46 & 2.26 & S & unknown \\
13-SN-109 & MBR148.22.532N & 1:46:09.34 & -67:28:00.1 & 6595.66504 & 19.22 & 5535 & Ia & 0.99 & Ia & 0.088 & 5537 & 3.70 & 6.02 & 3.71 & 12.70 & S & Ia \\
13-SN-110 & SMC801.19.64N & 0:59:40.13 & -65:04:57.2 & 6600.60124 & 18.84 & 5581 & Ia & 0.90 & - & - & - & (2.1) & - & - & - & - & Ia \\
13-SN-111 & SMC765.15.1578 & 23:42:18.27 & -67:39:38.8 & 6604.52732 & 19.78 & 5581 & Ia & 1.00 & - & - & - & 1.04 & - & 2.34 & 3.52 & S & Ia \\
13-SN-112 & LMC519.30.237N & 5:29:47.48 & -65:44:13.7 & 6608.84498 & 19.00 & 5581 & IIp & 0.48 & - & - & - & - & - & - & - & S & IIn \\
13-SN-113 & LMC550.07.4184 & 5:44:32.80 & -73:32:08.1 & 6607.80106 & 19.96 & 5581 & IIp & 0.70 & - & - & - & 0.60 & - & 1.10 & 1.31 & S & unknown \\
13-SN-114 & SMC700.19.63N & 0:19:35.61 & -69:24:12.5 & 6609.51537 & 19.45 & 5581 & Ia & 0.99 & - & - & - & 2.29 & - & 2.65 & 3.51 & S & Ia \\
13-SN-115 & MBR126.32.2978N & 3:00:56.46 & -70:16:47.9 & 6610.68031 & 19.78 & 5581 & IIp & 0.53 & - & - & - & - & - & - & - & S & unknown \\
13-SN-116 & MBR167.02.21N & 3:05:37.43 & -79:16:57.8 & 6610.63029 & 19.07 & 5581 & Ia & 0.32 & - & - & - & 2.01 & - & 2.02 & 3.82 & Ell & Ia \\
13-SN-117 & LMC640.28.6330 & 5:21:53.08 & -74:55:42.7 & 6614.83575 & 18.12 & 5608 & IIn & 0.67 & - & - & - & 1.16 & - & 1.43 & 2.42 & S & Ia \\
13-SN-118 & LMC505.24.64N & 5:14:47.50 & -66:50:29.1 & 6617.72346 & 19.01 & 5608 & Ia & 1.00 & Ia & 0.07 & 5595 & 6.18 & 8.16 & 6.81 & 2.75 & S & Ia \\
13-SN-119 & LMC566.28.27N & 6:19:45.55 & -71:20:19.4 & 6617.73597 & 19.98 & 5608 & IIp & 0.42 & - & - & - & - & - & - & - & Ell & DN \\
13-SN-120 & LMC556.29.2646 & 5:41:49.26 & -65:13:05.4 & 6618.81650 & 18.95 & 5608 & Ia & 0.90 & Ia & 0.07 & 5595 & - & - & - & - & S & Ia \\
13-SN-121 & LMC616.26.2478 & 4:22:42.87 & -68:16:34.2 & 6618.72813 & 21.17 & 5608 & IIp & 0.42 & - & - & - & 9.21 & - & 9.25 & 7.24 & S & unknown \\
13-SN-122 & LMC620.21.311 & 4:14:53.34 & -63:58:35.1 & 6618.73757 & 21.16 & 5608 & IIp & 0.70 & - & - & - & 0.04 & - & 0.04 & 1.22 & S & unknown \\
13-SN-123 & LMC604.05.69N & 5:58:30.38 & -63:33:38.3 & 6616.78872 & 18.36 & 5608 & IIn & 0.67 & Ia & 0.08 & 5602 & 0.16 & 0.23 & 0.16 & 1.99 & Ell & Ia \\
13-SN-124 & MBR201.19.51N & 3:08:52.84 & -69:25:09.7 & 6622.68027 & 20.22 & 5608 & Ia & 0.90 & Ia & 0.13 & 5615 & (29.6) & - & - & - & - & Ia \\
13-SN-125 & LMC621.26.1477N & 4:30:02.84 & -63:11:29.9 & 6622.74714 & 19.94 & 5608 & Ia & 0.90 & - & - & - & 12.53 & - & 12.53 & 2.75 & S & Ia \\
13-SN-126 & LMC620.18.111N & 4:19:47.17 & -63:43:21.6 & 6622.74502 & 19.15 & 5608 & Ia & 1.00 & Ia & 0.06 & 5615 & - & - & - & - & - & Ia \\
13-SN-127 & MBR203.11.294 & 3:05:57.62 & -67:08:18.5 & 6622.68470 & 20.74 & 5608 & Ia & 0.94 & - & - & - & 1.02 & - & 1.02 & 1.41 & S & Ia \\
13-SN-128 & LMC636.05.3425 & 4:59:42.75 & -75:18:04.8 & 6623.79520 & 19.24 & 5608 & IIp & 0.48 & - & - & - & 2.09 & - & 2.45 & 3.95 & S & Unknown/IIP \\
13-SN-129 & SMC787.06.77N & 0:16:41.97 & -66:16:07.4 & 6625.56369 & 19.45 & 5663 & Ia & 0.99 & Ia & 0.08 & 5622 & 11.54 & 17.20 & 11.81 & 4.92 & S & Ia \\
13-SN-130 & LMC615.28.29N & 6:36:46.99 & -68:52:22.4 & 6627.85385 & 19.65 & 5663 & IIp & 0.48 & Ia-pec & 0.09 & 5620 & - & - & - & - & S & Ia-pec \\
13-SN-131 & MBR149.05.146N & 1:43:36.96 & -66:50:39.7 & 6629.62253 & 19.48 & 5663 & Ia & 0.90 & - & - & - & 4.03 & 4.62 & 5.82 & 4.82 & S & Unknown \\
13-SN-132 & LMC612.26.1546N & 6:34:30.72 & -70:40:00.3 & 6635.81133 & 19.69 & 5663 & Ia & 1.00 & - & - & - & 5.53 & - & 5.54 & 3.45 & S & Ia \\
13-SN-133 & LMC560.22.309N & 5:57:43.83 & -69:50:06.2 & 6636.81928 & 19.43 & 5663 & IIp & 0.90 & - & - & - & - & - & - & - & S & IIp \\
13-SN-134 & LMC565.24.54N & 6:13:58.04 & -72:58:24.9 & 6636.81237 & 18.85 & 5663 & Ia & 0.90 & Ic-pec & 0.039 & 5696 & - & - & - & - & S & Ic-pec \\
13-SN-135 & MBR168.20.211N & 3:06:48.20 & -77:24:28.4 & 6636.60643 & 19.22 & 5663 & IIp & 0.92 & II & 0.057 & 5718 & 3.46 & 3.77 & 3.52 & 3.08 & S & IIP \\
13-SN-136 & LMC582.05.55N & 4:55:46.85 & -64:51:20.4 & 6639.75154 & 19.33 & 5663 & Ia & 1.00 & Ia & 0.080 & 5696 & 4.42 & 6.60 & 10.70 & 8.99 & S & Ia \\
13-SN-137 & MBR108.05.107N & 2:03:34.72 & -73:36:22.7 & 6639.60394 & 19.14 & 5663 & IIp & 0.48 & IIn & 0.075 & 5686 & 5.85 & 8.23 & 6.73 & 6.49 & S & IIn \\
13-SN-138 & SMC729.32.3036N & 1:19:02.87 & -68:13:14.7 & 6638.56148 & 18.59 & 5663 & IIn & 0.94 & IIn & 0.115 & 5683 & - & - & - & - & S & IIn \\
13-SN-139 & LMC677.15.55N & 8:09:25.36 & -70:37:59.3 & 6640.84276 & 20.07 & 5663 & Ia & 1.00 & - & - & - & 3.38 & - & 3.39 & 2.26 & S & Ia \\
13-SN-140 & LMC636.21.5988 & 5:02:52.42 & -74:40:11.3 & 6639.71997 & 20.20 & 5663 & IIp & 0.70 & - & - & - & 0.01 & - & 0.01 & 0.43 & - & Ia \\
13-NOVA-03 & MBR115.04.1856 & 2:26:43.16 & -76:34:37.8 & 6637.60535 & 17.15 & - & CN & 0.80 & - & - & - & - & - & - & - & - & CN \\
13-SN-141 & MBR171.15.67 & 3:16:00.60 & -77:05:38.5 & 6640.62861 & 18.96 & 5663 & Ia & 0.90 & Ia & 0.05 & 5696 & 0.09 & 0.08 & 0.23 & 5.05 & S & Ia \\
13-SN-142 & MBR162.24.72N & 2:10:37.64 & -78:01:50.2 & 6640.58723 & 19.34 & 5697 & Ia & 0.90 & - & - & - & 3.87 & - & 4.58 & 4.62 & S & Ia \\
13-SN-143 & LMC657.11.2388 & 6:37:30.46 & -76:45:00.1 & 6645.76906 & 20.56 & 5697 & Ia & 0.88 & - & - & - & 1.60 & - & 1.63 & 1.80 & S & Ia \\
13-SN-144 & LMC511.15.104N & 5:00:57.18 & -67:44:25.7 & 6647.74442 & 18.76 & 5697 & Ia & 1.00 & II & 0.04 & 5696 & - & - & - & - & S & IIP/IIL \\
13-SN-145 & LMC547.20.284N & 4:30:38.05 & -67:54:31.2 & 6647.70245 & 19.80 & 5697 & Ia & 0.80 & - & - & - & 9.17 & - & 9.22 & 3.50 & S & unknown \\
13-SN-146 & LMC548.11.58N & 4:33:00.74 & -67:05:21.5 & 6647.70467 & 18.69 & 5697 & Ia & 1.00 & - & - & - & - & - & - & - & S & Ia \\
13-SN-147 & LMC563.07.67N & 5:48:57.86 & -66:40:15.7 & 6649.78517 & 19.06 & 5697 & IIp & 0.48 & Ia-pec & 0.099 & 5689 & 0.08 & 0.14 & 0.09 & 6.57 & S & Ia-pec \\
13-SN-148 & LMC658.10.39N & 6:38:06.94 & -75:43:36.6 & 6652.70473 & 19.78 & 5697 & Ia & 1.00 & Ia & 0.043 & 5701 & - & - & - & - & S & Ia \\
13-SN-149 & LMC708.12.33N & 5:27:36.13 & -54:04:25.2 & 6653.59944 & 20.02 & 5709 & Ia & 1.00 & II & 0.079 & 5720 & 6.34 & 9.34 & 6.38 & 4.58 & S & IIn \\
13-SN-150 & LMC504.30.333N & 5:17:28.40 & -67:33:29.7 & 6654.76446 & 20.15 & 5709 & Ia & 0.90 & - & - & - & - & - & - & - & Ell & Ia \\
13-SN-151 & LMC517.28.304N & 5:34:24.69 & -68:10:07.8 & 6654.77073 & 20.08 & 5709 & IIp & 0.92 & - & - & - & - & - & - & - & S & Ia \\
13-SN-152 & MBR134.03.729N & 3:33:38.89 & -75:21:16.8 & 6656.64804 & 19.20 & 5709 & Ia & 0.90 & - & - & - & - & - & - & - & S & IIp \\
13-SN-153 & SMC792.28.83N & 0:34:37.69 & -64:42:10.1 & 6656.53603 & 18.75 & 5709 & Ia & 1.00 & - & - & - & 2.43 & - & 3.61 & 3.21 & S & Ia \\
13-SN-154 & LMC654.04.36N & 6:14:28.06 & -75:23:53.3 & 6657.67448 & 20.49 & 5709 & IIn & 0.51 & - & - & - & 0.13 & - & 0.13 & 1.11 & S & unknown \\
13-SN-155 & LMC669.10.39N & 7:35:27.88 & -71:15:07.1 & 6657.84450 & 20.45 & 5709 & Ia & 0.71 & - & - & - & 2.38 & - & 2.40 & 2.06 & - & IIp or IIn \\
13-SN-156 & LMC583.15.1914 & 4:54:08.66 & -63:15:37.1 & 6657.80890 & 20.31 & 5709 & Ia & 0.90 & Ia & 0.14 & 5716 & 0.03 & 0.08 & 0.07 & 1.73 & S & Ia \\
14-SN-001 & LMC664.05.78N & 7:02:35.58 & -72:48:15.9 & 6659.75454 & 19.07 & 5817 & Ia & 0.32 & CV & 0 & 5718 & - & - & - & - & S & DN \\
14-SN-002 & MBR231.04.42N & 4:04:31.71 & -63:50:15.6 & 6660.72357 & 19.53 & 5817 & Ia & 0.90 & Ia & 0.10 & 5748 & 2.75 & 5.01 & 3.34 & 4.90 & S & Ia \\
14-SN-003 & MBR108.19.69N & 2:09:59.06 & -73:02:11.8 & 6664.62577 & 19.10 & 5817 & IIp & 0.48 & - & - & - & 3.23 & - & 3.73 & 2.34 & S & unknown \\
14-SN-004 & LMC549.18.139N & 4:38:36.94 & -65:31:29.8 & 6668.76158 & 18.79 & 5817 & IIp & 0.92 & IIP & 0.03 & 5912 & 6.08 & 3.60 & 6.12 & 6.28 & S & IIP \\
14-SN-005 & LMC665.32.967 & 7:12:06.72 & -70:07:13.2 & 6682.73417 & 21.60 & 5817 & Ia & 0.97 & - & - & - & 0.21 & - & 0.25 & 6.82 & S & unknown \\
14-SN-006 & LMC671.21.46N & 7:45:41.68 & -70:18:58.4 & 6682.74720 & 19.87 & 5817 & IIp & 1.00 & - & - & - & 0.07 & - & 0.10 & 1.84 & S & IIp \\
14-SN-007 & MBR117.07.95N & 2:29:31.88 & -72:14:03.7 & 6690.54118 & 19.04 & 5875 & Ia & 0.99 & - & - & - & (1.8) & - & - & - & - & unknown \\
14-SN-008 & LMC578.23.56N & 5:05:52.96 & -63:44:54.4 & 6693.70282 & 19.52 & 5875 & Ia & 1.00 & - & - & - & 10.59 & - & 10.63 & 3.75 & AGN & unknown \\
14-SN-009 & LMC708.18.143N & 5:29:53.65 & -53:53:16.6 & 6694.74193 & 19.57 & 5875 & Ia & 1.00 & II & 0.056 & 5864 & 1.46 & 1.57 & 1.55 & 6.28 & S & Unknown \\
14-SN-010 & LMC614.07.2860 & 6:25:23.80 & -68:34:20.3 & 6694.77028 & 18.95 & 5875 & Ia & 1.00 & Ia & 0.081 & 5864 & 0.08 & 0.12 & 0.08 & 0.99 & - & Ia \\
14-SN-011 & LMC659.30.53N & 6:46:58.87 & -69:57:24.8 & 6695.72994 & 19.89 & 5875 & IIp & 0.70 & IIn & 0.083 & 5908 & 0.81 & 1.25 & 1.34 & 1.72 & S & IIn \\
14-SN-012 & LMC668.31.940N & 7:27:43.39 & -69:20:35.0 & 6695.74927 & 20.24 & 5875 & IIn & 0.51 & - & - & - & - & - & - & - & - & Unknown/IIP \\
14-SN-013 & LMC673.32.2006N & 7:40:35.37 & -72:28:17.1 & 6695.76024 & 20.17 & 5875 & Ia & 1.00 & - & - & - & - & - & - & - & - & Ia \\
14-SN-014 & LMC522.21.92N & 4:27:23.75 & -74:42:11.1 & 6698.66286 & 18.91 & 5875 & IIp & 0.90 & Ib & 0.05 & 5891 & 6.17 & 5.96 & 6.43 & 5.60 & S & Ib-unknown \\
14-SN-015 & LMC610.19.3006 & 6:25:23.80 & -68:34:20.3 & 6700.70514 & 18.98 & 5916 & Ia & 1.00 & - & - & - & - & - & - & - & - & Ia \\
14-SN-016 & LMC673.31.1107N & 7:42:01.43 & -72:29:41.4 & 6706.74447 & 19.41 & 5916 & Ia & 1.00 & Ia & 0.07 & 5908 & - & - & - & - & S & Ia \\
14-SN-017 & MBR218.07.74N & 3:30:32.38 & -63:43:16.1 & 6709.61149 & 19.07 & 5916 & Ia & 1.00 & - & - & - & - & - & - & - & AGN & Ia \\
14-SN-018 & LMC608.19.61N & 6:18:20.35 & -66:01:08.0 & 6710.70753 & 18.37 & 5916 & IIn & 0.67 & II & 0.03 & 5915 & - & - & - & - & S & IIP \\
14-SN-019 & LMC609.07.75N & 6:13:48.04 & -67:55:15.0 & 6710.70958 & 17.41 & 5916 & Ia & 1.00 & Ia & 0.04 & 5915 & 0.52 & 0.41 & 0.67 & 7.41 & Ell & Ia \\
14-SN-020 & LMC577.21.2359 & 6:24:30.22 & -73:58:10.6 & 6710.63295 & 20.27 & 5916 & IIp & 0.70 & II & 0.076 & 5934 & 0.04 & 0.06 & 0.09 & 0.82 & S & IIP \\
14-SN-021 & LMC555.18.230N & 5:48:23.49 & -66:47:29.7 & 6712.66078 & 17.92 & 5916 & Ia & 1.00 & Ia & 0.039 & 5919 & 2.80 & 2.14 & 3.20 & 2.21 & S & Ia \\
14-SN-022 & MBR145.13.195N & 4:03:27.76 & -72:11:27.0 & 6728.57155 & 17.10 & - & IIn & 0.67 & IIn & 0.024 & 5934 & 7.13 & 3.40 & 7.38 & 4.83 & S & IIn \\
14-SN-023 & LMC680.22.414N & 8:26:16.27 & -69:52:21.5 & 6715.73155 & 18.98 & - & DN & 1.00 & CV & 0 & 5937 & - & - & - & - & - & DN \\
14-SN-024 & LMC647.02.50N & 6:01:15.38 & -78:18:21.7 & 6719.64051 & 19.69 & - & IIp & 0.48 & Ia & 0.1 & 5938 & - & - & - & - & S & Ia \\
14-SN-025 & LMC689.24.78N & 5:07:07.33 & -54:57:24.6 & 6721.58127 & 20.34 & - & Ia & 1.00 & - & - & - & 1.55 & - & 2.10 & 2.74 & S & Ia \\
14-SN-026 & LMC697.18.174N & 5:22:13.47 & -56:46:47.6 & 6721.55699 & 20.10 & - & IIp & 0.70 & - & - & - & 2.13 & - & 2.37 & 5.15 & S & IIp \\
14-SN-027 & MBR164.04.58N & 2:41:49.91 & -78:24:41.8 & 6728.51211 & 18.62 & - & IIn & 0.41 & - & - & - & 0.94 & - & 0.94 & 2.41 & S & unknown \\
14-SN-028 & LMC635.01.33N & 5:09:42.76 & -76:41:29.6 & 6734.55975 & 20.17 & - & - & - & - & - & - & 0.40 & - & 0.46 & 2.58 & Ell & - \\
14-NOVA-01 & BLG643.22.8N & 17:55:20.27 & -23:23:54.5 & 6735.89972 & 16.29 & - & - & - & - & - & - & - & - & - & - & - & - \\
